3D Shape Segmentation with Geometric Deep Learning

The semantic segmentation of 3D shapes with a high-density of vertices could be impractical due to large memory requirements. To make this problem computationally tractable, we propose a neural-network based approach that produces 3D augmented views of the 3D shape to solve the whole segmentation as sub-segmentation problems. 3D augmented views are obtained by projecting vertices and normals of a 3D shape onto 2D regular grids taken from different viewpoints around the shape. These 3D views are then processed by a Convolutional Neural Network to produce a probability distribution function (pdf) over the set of the semantic classes for each vertex. These pdfs are then re-projected on the original 3D shape and postprocessed using contextual information through Conditional Random Fields. We validate our approach using 3D shapes of publicly available datasets and of real objects that are reconstructed using photogrammetry techniques. We compare our approach against state-of-the-art alternatives.

==> resources/arch.tex <==
\begin{tikzpicture}[
	node distance=2cm, 
	>=stealth',
	views/.style={
		shape=rectangle, 
        rounded corners,
		fill=black!5,
		draw=black!20, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center
	},
	input/.style={
		shape=rectangle, 
        rounded corners,
		fill=black!25!green!10,
		draw=black!25!green!40, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center
	},
	params/.style={
		shape=rectangle, 
		rounded corners,
		fill=blue!15,
		draw=blue!40, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center
	},
	output/.style={
		shape=rectangle, 
		rounded corners,
		fill=red!10,
		draw=red!40, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center
	},
	arrow/.style={
		-latex,
		color=black,
		draw=black,
		font=\fontsize{8}{8}\selectfont
	}
]
	
% blocks
\node[views] (S) {$S$};
\coordinate[right = 0.25 cm of S] (V_);
\coordinate[above = 2 cm of V_] (V1_);
\node[views, right = 0.33 cm of  V1_] (V1) {$v_1$};
\coordinate[above = 1 cm of V_] (V2_);
\node[views, right = 0.33 cm of  V2_] (V2) {$v_2$};
\coordinate[below = 1 cm of V_] (Vn_);
\node[views, right = 0.33 cm of  Vn_] (Vn) {$v_n$};
\coordinate[below = 3.5 cm of V_] (L_);
\node[views, right = 0.33 cm of  L_] (L) {$g$};
%
\coordinate[right = 1.2 cm of V1_] (I1_);
\coordinate[above = 0.5 cm of I1_] (I11_);
\coordinate[below = 0.5 cm of I1_] (I12_);
\coordinate[below = 1.5 cm of I1_] (I13_);
\node[input, right = 0.33 cm of  I11_] (I11) {$x_1$};
\node[input, right = 0.33 cm of  I12_] (I12) {$M_1$};
\node[input, right = 0.33 cm of  I13_] (I13) {$i_1$};
\coordinate[right = 1.33 cm of I11_] (N11_);
\coordinate[right = 1.33 cm of I12_] (N12_);
\coordinate[right = 1.33 cm of I1_] (N1_);
\node[params, right = 0.33 cm of N1_] (N1) {$\textrm{Net}$};
\node[output, right = 0.33 cm of N1] (O1) {$y_1$};
\coordinate[right = 3.75 cm of I1_] (O11_);
\coordinate[right = 3.75 cm of I13_] (O12_);
%
\coordinate[right = 1.2 cm of Vn_] (In_);
\coordinate[above = 0.5 cm of In_] (In1_);
\coordinate[below = 0.5 cm of In_] (In2_);
\coordinate[below = 1.5 cm of In_] (In3_);
\node[input, right = 0.33 cm of  In1_] (In1) {$x_n$};
\node[input, right = 0.33 cm of  In2_] (In2) {$M_n$};
\node[input, right = 0.33 cm of  In3_] (In3) {$i_n$};
\coordinate[right = 1.33 cm of In1_] (Nn1_);
\coordinate[right = 1.33 cm of In2_] (Nn2_);
\coordinate[right = 1.33 cm of In_] (Nn_);
\node[params, right = 0.33 cm of Nn_] (Nn) {$\textrm{Net}$};
\node[output, right = 0.33 cm of Nn] (On) {$y_n$};
\coordinate[right = 3.75 cm of In_] (On1_);
\coordinate[right = 3.75 cm of In3_] (On2_);
%
\coordinate[below = 0.75 cm of O11_] (P1_);
\coordinate[below = 0.75 cm of On1_] (P2_);
\node[params, right = 0.33 cm of P1_] (P) {$\textrm{Proj}$};
\node[output, right = 0.33 cm of P] (C) {$\hat{y}$};
%
\coordinate[right = 0.25 cm of C] (C11_);
\coordinate[right = 7.415 cm of L_] (C12_);
\coordinate[below = 1 cm of C11_] (C1_);
\node[params, right = 0.33 cm of C1_] (C1) {$\textrm{CRF}$};
\node[output, right = 0.33 cm of C1] (Y) {$\bar{y}$};

% arrows
\draw [-] (S.east) -- (V_);
\draw [-] (V_) -- (V1_);
\draw [arrow] (V1_) -- (V1);
\draw [-] (V_) -- (V2_);
\draw [arrow] (V2_) -- (V2);
\draw [-] (V_) -- (Vn_);
\draw [arrow] (Vn_) -- (Vn);
\draw [-] (V_) -- (L_);
\draw [arrow] (L_) -- (L);
%
\draw [-] (V1) -- (I1_);
\draw [-] (I1_) -- (I11_);
\draw [-] (I1_) -- (I12_);
\draw [-] (I1_) -- (I13_);
\draw [arrow] (I11_) -- (I11);
\draw [arrow] (I12_) -- (I12);
\draw [arrow] (I13_) -- (I13);
\draw [-] (I11) -- (N11_);
\draw [-] (I12) -- (N12_);
\draw [-] (N11_) -- (N1_);
\draw [-] (N12_) -- (N1_);
\draw [arrow] (N1_) -- (N1);
\draw [arrow] (N1) -- (O1);
\draw [-] (O1) -- (O11_);
\draw [-] (I13) -- (O12_);
%
\draw [-] (Vn) -- (In_);
\draw [-] (In_) -- (In1_);
\draw [-] (In_) -- (In2_);
\draw [-] (In_) -- (In3_);
\draw [arrow] (In1_) -- (In1);
\draw [arrow] (In2_) -- (In2);
\draw [arrow] (In3_) -- (In3);
\draw [-] (In1) -- (Nn1_);
\draw [-] (In2) -- (Nn2_);
\draw [-] (Nn1_) -- (Nn_);
\draw [-] (Nn2_) -- (Nn_);
\draw [arrow] (Nn_) -- (Nn);
\draw [arrow] (Nn) -- (On);
\draw [-] (On) -- (On1_);
\draw [-] (In3) -- (On2_);
%
\draw [-] (O11_) -- (O12_);
\draw [-] (On1_) -- (On2_);
\draw [arrow] (P1_) -- (P);
\draw [arrow] (P2_) -- (P.south);
\draw [arrow] (P) -- (C);
% 
\draw [-] (C) -- (C11_);
\draw [-] (L) -- (C12_);
\draw [-] (C11_) -- (C12_);
\draw [arrow] (C1_) -- (C1);
\draw [arrow] (C1) -- (Y);

% regions
%\begin{scope}[on background layer]
%\node[draw, rectangle, inner sep=7pt, rounded corners,fit={(CONV1) (FC1)}, fill=blue!10] (fit) {};
%\end{scope}
%\node[below right, inner sep=5pt] at (fit.south west) {$g_1$};

\end{tikzpicture}


==> resources/crf_net.tex <==
%\begin{filecontents}{crf_net.tikz}
\begin{tikzpicture}[
	node distance=2cm, 
	>=stealth',
	fixed/.style={
		shape=rectangle, 
        rounded corners,
		fill=black!5,
		draw=black!20, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center
	},
	input/.style={
		shape=rectangle, 
        rounded corners,
		fill=black!25!green!10,
		draw=black!25!green!40, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center
	},
	param/.style={
		shape=rectangle, 
		rounded corners,
		fill=blue!15,
		draw=blue!40, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center
	},
	output/.style={
		shape=rectangle, 
		rounded corners,
		fill=black!20!red!10,
		draw=black!20!red!40, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center
	},
	feat/.style={
		shape=rectangle, 
		rounded corners,
		fill=black!15!yellow!15,
		draw=black!15!orange!30, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center
	},
	oper/.style={
		shape=rectangle,
		rounded corners,
		fill=white!15, 
		draw=black!40, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center, 
	},
	arrow/.style={
		-latex,
		color=black,
		draw=black,
		font=\fontsize{8}{8}\selectfont
	}
]

% blocks
\coordinate (A0);
\node[fixed, right = 4.1mm of A0] (A1) {$\tilde{\textbf{p}}$};
\node[oper, right = 3.3mm of A1] (A2) {$\log(\cdot)$};
\node[input, right = 3.3mm of A2] (A3) {$\textbf{u}$};

\node[fixed, below = 5.5mm of A0] (B1) {$\textbf{d}_{\footnotesize \textrm{geod}}$};
\coordinate[right = 0.75mm of B1] (B2);
\node[oper, right = 3.3mm of B2] (B3) {$\phi_{\footnotesize \textrm{near}}( \cdot )$};
\node[input, right = 3.3mm of B3] (B4) {$\textbf{k}_{\footnotesize \textrm{near}}$};

\coordinate[below = 9.75mm of B2] (C2);
\node[oper, right = 3.3mm of C2] (C3) {$\phi_{\footnotesize \textrm{far}}( \cdot )$};
\node[input, right = 5.4mm of C3] (C4) {$\textbf{k}_{\footnotesize \textrm{far}}$};

\node[fixed, below = 13mm of B1] (D1) {$\textbf{d}_{\footnotesize \textrm{feat}}$};
\node[oper, right = 3.3mm of D1] (D3) {$\phi_{\footnotesize \textrm{feat}}( \cdot )$};
\node[input, right = 5.4mm of D3] (D4) {$\textbf{k}_{\footnotesize \textrm{feat}}$};

\node[inner sep=-0.5pt, right = 41.75mm of A1] (E1) {$\bullet$};
\node[oper, below = 5mm of E1] (E2) {$\sigma(\cdot)$};
\node[feat, right = 10mm of C4] (E3) {$\textbf{p}^{(1)}$};

\node[feat, right = 23mm of B4] (B5) {$\textbf{p}^{(2)}$};
\node[feat, right = 25mm of C4] (C5) {$\textbf{p}^{(3)}$};
\node[feat, right = 23.7mm of D4] (D5) {$\textbf{p}^{(4)}$};

\node[param, right = 7.5mm of B5] (B6) {$\textbf{W}_{\footnotesize \textrm{near}}$};
\node[param, right = 7.5mm of C5] (C6) {$\textbf{W}_{\footnotesize \textrm{far}}$};
\node[param, right = 7.5mm of D5] (D6) {$\textbf{W}_{\footnotesize \textrm{feat}}$};

\node[feat, right = 3.3mm of B6] (B7) {$\textbf{p}^{(5)}$};
\node[feat, right = 5.45mm of C6] (C7) {$\textbf{p}^{(6)}$};
\node[feat, right = 4.1mm of D6] (D7) {$\textbf{p}^{(7)}$};

\coordinate[right = 3.3mm of B7] (B8);

\coordinate[below = 1.5mm of B7] (F1);
\node[oper, circle, inner sep=1.25pt, right = 8mm of F1] (F2) {$-$};
\node[feat, right = 2.3mm of F2] (F3) {$\textbf{p}^{(8)}$};
\node[oper, circle, inner sep=1.25pt, right = 13.1mm of D7] (F4) {$+$};

\coordinate[below = 2.5mm of F4] (F5);
\coordinate[left = 49mm of F5] (F6);
\coordinate[below = 5mm of F6] (G1);
\node[feat, right = 3.3mm of G1] (G2) {$\textbf{p}^{(9)}$};
\node[param, right = 7.5mm of G2] (G3) {$\textbf{W}_{\footnotesize \textrm{comp}}$};
\node[feat, right = 3.3mm of G3] (G4) {$\textbf{p}^{(10)}$};
\node[oper, circle, inner sep=1.25pt, right = 3.3mm of G4] (G5) {$-$};
\coordinate[right = 74.5mm of E1] (G6);
\node[feat, right = 2.5mm of G5] (G7) {$\textbf{p}^{(11)}$};
\node[inner sep=-0.5pt, right = 1mm of G7] (G8) {$\bullet$};

\coordinate[above = 41mm of G8] (G9);
\coordinate[left = 91.5mm of G9] (G10); 
\node[rotate=90, above = 21.5mm of G8] {\footnotesize if $i=1, \dots, n_{\footnotesize \textrm{iter}}-1$};
\coordinate[below = 9mm of G8] (G11); 
\node[output, left = 17mm of G11] (G12) {$\textbf{y}$}; 

% arrows
\draw[arrow] (A1) -- (A2);
\draw[arrow] (A2) -- (A3);
\draw[-] (B1) -- (B2);
\draw[arrow] (B2) -- (B3);
\draw[arrow] (B3) -- (B4);
\draw[-] (B2) -- (C2);
\draw[arrow] (C2) -- (C3);
\draw[arrow] (C3) -- (C4);
\draw[arrow] (D1) -- (D3);
\draw[arrow] (D3) -- (D4);

\draw[arrow] (B4.east) -- (E3.west) node[oper, circle, inner sep=1.5pt, midway] {$\bullet$};
\draw[arrow] (C4.east) -- (E3.west) node[oper, circle, inner sep=1.5pt, midway] {$\bullet$};
\draw[arrow] (D4.east) -- (E3.west) node[oper, circle, inner sep=1.5pt, midway] {$\bullet$};

\draw[-] (A3) -- (E1);
\draw[arrow] (E1) -- (E2);
\draw[arrow] (E2) -- (E3);

\draw[arrow] (E3.east) -- (B5.west);
\draw[arrow] (E3.east) -- (C5.west);
\draw[arrow] (E3.east) -- (D5.west);

\draw[arrow] (B5.east) -- (B6.west) node[oper, circle, inner sep=1.5pt, pos=0.39] {$\bullet$};
\draw[arrow] (C5.east) -- (C6.west) node[oper, circle, inner sep=1.5pt, pos=0.39] {$\bullet$};
\draw[arrow] (D5.east) -- (D6.west) node[oper, circle, inner sep=1.5pt, pos=0.39] {$\bullet$};

\draw[arrow] (B6) -- (B7);
\draw[arrow] (C6) -- (C7);
\draw[arrow] (D6) -- (D7);

\draw[arrow] (B7.east) -- (F2.west);
\draw[arrow] (C7.east) -- (F2.west);
\draw[arrow] (F2) -- (F3);
\draw[arrow] (F3) -- (F4);
\draw[arrow] (D7) -- (F4);

\draw[-] (F4) -- (F5);
\draw[-] (F5) -- (F6);
\draw[-] (F6) -- (G1);
\draw[arrow] (G1) -- (G2);
\draw[arrow] (G2.east) -- (G3.west) node[oper, circle, inner sep=1.5pt, pos=0.4] {$\bullet$};
\draw[arrow] (G3) -- (G4);
\draw[arrow] (G4) -- (G5);
\draw[-] (E1) -- (G6);
\draw[arrow] (G6) -- (G5);
\draw[arrow] (G5) -- (G7);
\draw[-] (G7) -- (G8);

\draw[-] (G8) -- (G9);
\draw[-] (G9) -- (G10);
\draw[arrow] (G10) -- (E2.north -| G10.south);

\draw[-] (G8) -- (G11);
\draw[arrow] (G11) -- (G12) node[above, midway] {if $i=n_{\footnotesize \textrm{iter}}$};

% regions
\coordinate[left = 11.5mm of G10] (TL);
\coordinate[below right = 1.5mm of G8] (BR);
\begin{scope}[on background layer]
\node[
	draw, 
	rectangle, 
	inner sep=7pt, 
	rounded corners, 
	fit={(TL) (BR)}, 
	fill=blue!5,
	draw=blue!30
	] (fit) {};
\end{scope}
\coordinate[below = 42mm of TL] (T);
\node[right = -1mm of T, blue!30] (TT) {CRF Net}; 

\end{tikzpicture}
%\end{filecontents}


==> resources/proj_net.tex <==
%\begin{filecontents}{proj_net.tikz}
\begin{tikzpicture}[
	node distance=2cm, 
	>=stealth',
	fixed/.style={
		shape=rectangle, 
            	rounded corners,
		fill=black!5,
		draw=black!20, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center
	},
	input/.style={
		shape=rectangle, 
            	rounded corners,
		fill=black!25!green!10,
		draw=black!25!green!40, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center
	},
	param/.style={
		shape=rectangle, 
		rounded corners,
		fill=blue!15,
		draw=blue!40, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center
	},
	output/.style={
		shape=rectangle, 
		rounded corners,
		fill=black!20!red!10,
		draw=black!20!red!40, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center
	},
	feat/.style={
		shape=rectangle, 
		rounded corners,
		fill=black!15!yellow!15,
		draw=black!15!orange!30, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center
	},
	arrow/.style={
		-latex,
		color=black,
		draw=black,
		font=\fontsize{8}{8}\selectfont
	}
]

% blocks
\node[input] (A1) {$\textbf{f}_1$};
\node[input, below = 2mm of A1] (B1) {$\textbf{i}_1$};
\node[fixed, right = 5mm of A1] (C1) {Proj Layer};
\coordinate[below = 4.65mm of C1.south] (D1);
\node[feat, right = 5mm of C1] (E1) {$\tilde{\textbf{g}}_1$};
%
\node[input, below = 12mm of A1] (A2) {$\textbf{f}_2$};
\node[input, below = 2mm of A2] (B2) {$\textbf{i}_2$};
\node[fixed, right = 5mm of A2] (C2) {Proj Layer};
\coordinate[below = 4.65mm of C2.south] (D2);
\node[feat, right = 5mm of C2] (E2) {$\tilde{\textbf{g}}_2$};
%
\node[below = 25.25mm of A1] (dots1) {$\vdots$};
\node[right = 15.75mm of dots1] (dots2) {$\vdots$};
\node[right = 35.5mm of dots1] (dots3) {$\vdots$};
%
\node[input, below = 35mm of A1] (An) {$\textbf{f}_N$};
\node[input, below = 2mm of An] (Bn) {$\textbf{i}_N$};
\node[fixed, right = 5mm of An] (Cn) {Proj Layer};
\coordinate[below = 4.65mm of Cn.south] (Dn);
\node[feat, right = 5mm of Cn] (En) {$\tilde{\textbf{g}}_N$};
%
\node[fixed, right = 5mm of E1] (F1) {Mean Layer};
\coordinate[right = 10mm of E2] (F2);
\coordinate[above = 14.25mm of F2] (F1_);
\coordinate[right = 16.5mm of En] (Fn);
%
\node[output, right = 5mm of F1] (G) {$\tilde{\textbf{g}}$};

% arrows
\draw[arrow] (A1.east) -- (C1);
\draw[-] (B1.east) -- (D1);
\draw[arrow] (D1) -- (C1);
\draw[arrow] (C1) -- (E1);
%
\draw[arrow] (A2.east) -- (C2);
\draw[-] (B2.east) -- (D2);
\draw[arrow] (D2) -- (C2);
\draw[arrow] (C2) -- (E2);
%
\draw[arrow] (An.east) -- (Cn);
\draw[-] (Bn.east) -- (Dn);
\draw[arrow] (Dn) -- (Cn);
\draw[arrow] (Cn) -- (En);
%
\draw[arrow] (E1) -- (F1);
\draw[-] (E2) -- (F2);
\draw[arrow] (F2) -- (F1_);
\draw[-] (En) -- (Fn);
\draw[arrow] (Fn) -- (F1);
%
\draw[arrow] (F1) -- (G);

% regions
\coordinate[above left = 1mm of C1] (TL);
\coordinate[below = 50mm of F1.east] (BR);
\begin{scope}[on background layer]
\node[
	draw, 
	rectangle, 
	inner sep=7pt, 
	rounded corners, 
	fit={(TL) (BR)}, 
	fill=blue!5,
	draw=blue!30
	] (fit) {};
\end{scope}
\node[right = 52mm of Bn, blue!30] (T) {Proj Net}; 

\end{tikzpicture}
%\end{filecontents}


==> resources/view_net.tex <==
%\begin{filecontents}{view_net.tikz}
\begin{tikzpicture}[
	node distance=2cm, 
	>=stealth',
	fixed/.style={
		shape=rectangle, 
        rounded corners,
		fill=black!5,
		draw=black!20, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center
	},
	input/.style={
		shape=rectangle, 
        rounded corners,
		fill=black!25!green!10,
		draw=black!25!green!40, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center
	},
	param/.style={
		shape=rectangle, 
		rounded corners,
		fill=blue!15,
		draw=blue!40, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center
	},
	output/.style={
		shape=rectangle, 
		rounded corners,
		fill=black!20!red!10,
		draw=black!20!red!40, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center
	},
	feat/.style={
		shape=rectangle, 
		rounded corners,
		fill=black!15!yellow!15,
		draw=black!15!orange!30, 
		text=black,
		font=\fontsize{12}{12}\selectfont,
		align=center
	},
	arrow/.style={
		-latex,
		color=black,
		draw=black,
		font=\fontsize{8}{8}\selectfont
	}
]

% blocks
\node[input] (Dn) {$\textbf{f}_i$};
\node[input, below = 4.7mm of Dn] (Ds) {$\textbf{P}_i$};
\node[inner sep=-0.5pt, right = 11.6mm of Ds] (Es) {$\bullet$};
%
\node[param, right = 5mm of Dn] (F) {$\textbf{W}_{\footnotesize \textrm{CONV}}^{(1)}$};
\node[feat, right = 5mm of F] (Fr) {$\textbf{g}_i^{(1)}$};
%
\node[param, right = 5mm of Fr] (G) {$\textbf{W}_{\footnotesize \textrm{CONV}}^{(2)}$};
\node[feat, right = 5mm of G] (Gr) {$\textbf{g}_i^{(2)}$};
\node[inner sep=-0.5pt, below = 6.2mm of G] (Gs) {$\bullet$};
%
\node[param, right = 5mm of Gr] (H) {$\textbf{W}_{\footnotesize \textrm{CONV}}^{(3)}$};
\node[feat, right = 5mm of H] (Hr) {$\textbf{g}_i^{(3)}$};
\node[inner sep=-0.5pt, below = 6.2mm of H] (Hs) {$\bullet$};
%
\node[param, below = 12.5mm of Hr] (I) {$\textbf{W}_{\footnotesize \textrm{FC}}^{(1)}$};
\node[feat, left = 5mm of I] (Il) {$\textbf{g}_i^{(4)}$};
\node[param, left = 5mm of Il] (J) {$\textbf{W}_{\footnotesize \textrm{FC}}^{(2)}$};
\node[feat, left = 5mm of J] (Jl) {$\textbf{g}_i^{(5)}$};
\node[param, left = 5mm of Jl] (K) {$\textbf{W}_{\footnotesize \textrm{FC}}^{(3)}$};
\node[feat, left = 5mm of K] (Kl) {$\textbf{g}_i^{(6)}$};
\node[fixed, left = 5mm of Kl] (L) {$\sigma(\cdot)$}; % softmax
\node[output, below = 3.8mm of Ds] (Ll) {$\textbf{g}_i$};

% arrows
\draw[arrow] (Dn) -- (F);
\draw[-] (Ds) -- (Es);
\draw[arrow] (Es) -- (F);
\draw[arrow] (F) -- (Fr);
\draw[arrow] (Fr) -- (G);
\draw[arrow] (G) -- (Gr);
\draw[-] (Es) -- (Gs);
\draw[arrow] (Gs) -- (G);
%
\draw[arrow] (Gr) -- (H);
\draw[arrow] (H) -- (Hr);
\draw[-] (Gs) -- (Hs);
\draw[arrow] (Hs) -- (H);
%
\draw[arrow] (Hr) -- (I);
\draw[arrow] (I) -- (Il);
\draw[arrow] (Il) -- (J);
\draw[arrow] (J) -- (Jl);
\draw[arrow] (Jl) -- (K);
\draw[arrow] (K) -- (Kl);
\draw[arrow] (Kl) -- (L);
\draw[arrow] (L) -- (Ll);

% regions
\coordinate[right = 5mm of Dn.north east] (TL1);
\coordinate[above = 5mm of TL1] (TL);
\coordinate[below right = 0mm of I] (BR);
\begin{scope}[on background layer]
\node[
	draw, 
	rectangle, 
	inner sep=7pt, 
	rounded corners, 
	fit={(TL) (BR)}, 
	fill=blue!5,
	draw=blue!30
	] (fit) {};
\end{scope}
\node[above = 4.75mm of Hr.west, blue!30] (T) {\hspace{3mm} View Net}; 

\end{tikzpicture}
%\end{filecontents}

